Mitigating the Backdoor Effect for Multi-Task Model Merging via Safety-Aware Subspace

Model merging has gained significant attention as a cost-effective approach to integrate multiple single-task fine-tuned models into a unified one that can perform well on multiple tasks. However, existing model merging techniques primarily focus on resolving conflicts between task-specific models, they often overlook potential security threats, particularly the risk of backdoor attacks in the open-source model ecosystem. In this paper, we first investigate the vulnerabilities of existing model merging methods to backdoor attacks, identifying two critical challenges: backdoor succession and backdoor transfer. To address these issues, we propose a novel Defense-Aware Merging (DAM) approach that simultaneously mitigates task interference and backdoor vulnerabilities. Specifically, DAM employs a meta-learning-based optimization method with dual masks to identify a shared and safety-aware subspace for model merging. These masks are alternately optimized: the Task-Shared mask identifies common beneficial parameters across tasks, aiming to preserve task-specific knowledge while reducing interference, while the Backdoor-Detection mask isolates potentially harmful parameters to neutralize security threats. This dual-mask design allows us to carefully balance the preservation of useful knowledge and the removal of potential vulnerabilities. Compared to existing merging methods, DAM achieves a more favorable balance between performance and security, reducing the attack success rate by 2-10 percentage points while sacrificing only about 1% in accuracy. Furthermore, DAM exhibits robust performance and broad applicability across various types of backdoor attacks and the number of compromised models involved in the merging process. Our codes and models are available at https://github.com/Yangjinluan/DAM.

==> section/1.introduction.tex <==
\begin{abstract}
  Model merging has gained significant attention as a cost-effective approach to integrate multiple single-task fine-tuned models into a unified one that can achieve good performance on multiple tasks. 
  However, existing model merging techniques primarily focus on facilitating the transfer and inheritance of useful knowledge through solving the conflict among tasks while overlooking the potential risks posed by harmful elements such as backdoors, which can be intentionally injected by adversaries during finetuning. 
  In this paper, we first revisit current model merging strategies and uncover critical challenges related to backdoor succession and backdoor transfer.
  Based on these findings, we propose a novel \emph{Defense-Aware Merging (DAM)} algorithm that utilizes a common, safety-aware subspace to concurrently address task interference and backdoor challenges for multi-task merging.
  Considering task vectors as representations of optimized directions within the model weight space for specific tasks, we present the following contributions:
  (1) Exposing Vulnerabilities in Model Merging. We are the first to systematically investigate the phenomena of backdoor succession and backdoor transfer in multi-task model merging; (2) Proposing Unified Safety-Performance Merging Algorithm. We introduce a novel algorithm that simultaneously addresses task interference and backdoor vulnerabilities during the model merging process; (3) Dual Mask Optimization. We develop a meta-learning-based optimization approach that employs two masks: one designed to identify a shared parameter subspace to mitigate task interference, while the other focuses on detecting parameters associated with potential backdoor threats. Subsequently, we reset the parameters within the full mask region to their pre-trained weights during the multi-task merging to develop a merged model that effectively balances performance and safety. We validate the effectiveness of DAM on several benchmarks and backbones, achieving a decrease in Attack Success Rate(ASR) by 2-10 scores while sacrificing only about 1 score in Accuracy(ACC) compared to existing state-of-the-art (SOTA) merging methods, thereby establishing a more favorable trade-off between safety and performance. Moreover, the consistently superior results independent of the type of backdoor or the number of backdoored models can emphasize the robustness and generalizability of our method. Our codes and models are available at:

  % Fine-tuning pre-trained models is crucial to enhancing their task-specific performance. Recently, to construct a unified model that performs well across tasks, model merging has achieved great attention as a new learning paradigm due to its great performance and cheap cost. Nevertheless, existing merging techniques mainly explore the strategies to facilitate the transfer and inheritance of knowledge by resolving potential conflicts among tasks. Exactly, apart from the useful knowledge, the harmful or unsafe part from one or more individual fine-tuned models (e.g. backdoor), which may be intentionally injected by the adversary, should also be considered carefully during merging. In this paper, we conduct extensive experiments to display two neglected but important phenomena related to the safety of merging: backdoor succession and backdoor transfer. To address these problems, we introduce a novel defense-aware merging (DAM) algorithm by identifying a shared and safe-aware subspace to mitigate the interference and backdoor issues simultaneously, aiming to achieve a good trade-off between performance and safety during merging. Compared with previous subspace-based merging methods, we additionally identify the backdoor-related parameters and reset them to the pre-trained weights, through synthesizing the universal perturbations for each task-specific model without any assumption about backdoor information. We conduct extensive experiments on several backbones and datasets to verify the effectiveness of DAM for multi-task merging. Moreover, the compared results with traditional post-defense methods show that DAM can also achieve comparable performance in mitigating the backdoor issues without the need for additional training. 

  % we propose novel defense-aware merging methods to identify a shared and safe subspace to mitigate the backdoor and interference issues simultaneously.


  % As it remains unclear whether existing merging methods can naturally cope with this neglected problem, this work aims to conduct extensive experiments to investigate this potential safety issue through analyzing the interaction effect between parameters of the clean model and backdoor model during merging with the following insights: \textbf{(1) Backdoor Succession:} The backdoor effect from one or more task-specific models can succeed during merging and influence the safety and performance of the merging model on the corresponding specific task even though adopting the state-of-the-art merging techniques; \textbf{(2) Backdoor Transfer:} The backdoor effect from backdoored task-specific models can transfer to other clean task-specific models during merging and influence the safety and performance of the merging model on tasks related to the clean models. 

  % To address these challenges, we propose a defense-aware merging (DAM) algorithm that can identify a common and safe subspace, which is then used to mitigate the backdoor and interference problems simultaneously. 

  % Experiments on several backbones and benchmarks can demonstrate the effectiveness of DAM compared with existing merging methods. Moreover, the comparison results with traditional post-defense methods can also illustrate that DAM can achieve comparable performance without additional training. The code and model are available at:
\end{abstract}

\section{Introduction}
% 第一段： abstract的第一句展开（background）
The rapid advancement of machine learning has led to the development of highly sophisticated models capable of performing a wide range of tasks with remarkable accuracy \citep{yang2024model}. Among these advancements, multi-task model merging has emerged as a pivotal technique, aiming to integrate the parameters of multiple single-task fine-tuned models into a unified one that excels across various tasks \citep{tang2024fusionbench}. This paradigm not only enhances task-specific performance but also offers computational efficiency and cost-effectiveness \citep{izmailov2018averaging, frankle2020linear, ilharco2022patching}.

% However, despite its promising potential, multi-task model merging faces significant challenges, particularly concerning the safety and security of the merged models.


% 第二段： abstract的第二句展开 （motivation）

Existing model merging techniques primarily concentrate on resolving conflicts among task-specific models to facilitate the smooth transfer and inheritance of useful knowledge. They often employ strategies such as gradient-conflict-based \citep{yadav2024ties} and subspace-based methods \citep{tang2023concrete, tam2024merging, yu2024language} to achieve this goal. Nevertheless, these approaches largely overlook the potential inclusion of harmful elements, such as backdoors, which can be intentionally injected by adversaries during fine-tuning \citep{wu2024backdoorbench}. Exactly, under the real share-and-play scenario \citep{liu2024lora},  people will download and fine-tune open-source large foundation models to enhance their performance for various downstream tasks and re-upload these fine-tuned models to open-source platforms (e.g. Huggingface) without releasing their training data. This makes it possible for adversaries to upload backdoored models to break the safeguard of the merging process, leading to potential risks while deploying previous multi-task merging algorithms for practical applications. Thus, some questions naturally arise:

\begin{center}
  \textbf{\emph{Whether existing multi-task merging methods have already coped with the neglected safety issues well? \\
      If not, how can we mitigate the backdoor effect for the multi-task merging better?}}
\end{center}

% 第三段： abstract的第三句展开（revisiting，放一个图）
In this paper, we first revisit current multi-task merging strategies and evaluate their performance and safety while utilizing the backdoored task-specific models for merging. We uncover two negative but critical issues: backdoor succession and backdoor transfer. Backdoor succession refers to the phenomenon where the harmful elements from backdoored task-specific models still persist in the merged model though adopting existing state-of-the-art (SOTA) merging methods, while backdoor transfer denotes the spread of these harmful elements from backdoored models to clean models during the merging process. Both of them pose the security risk of multi-task merging process, highlighting the urgent need for a safety-aware model merging approach that not only maximizes performance but also ensures the safety and security of the merged model.

% 第四段： abstract的第四，五句展开（solution and technical contribution


To address these challenges, we propose a novel Defense-Aware Merging (DAM) algorithm that concurrently mitigates interference and backdoor issues by leveraging the concept of a shared, safety-aware subspace. Specifically, for task vectors, which represent the optimized direction in the weight space of a pre-trained model on corresponding tasks, we develop a meta-learning-based optimization approach that employs two masks: one designed to identify a shared parameter subspace to mitigate task interference, while the other focuses on detecting parameters associated with potential backdoor threats. Subsequently, we reset the parameters within the full mask region of task vectors to their pre-trained weights to develop a merged model that effectively balances performance and safety.
% 第五段： abstract的第六句展开（performance gains很重要）
Experiments on several benchmarks and backbones are conducted to validate the effectiveness of DAM, which decreases the Attack Success Rate(ASR) by 2-10 scores with a minor sacrifice of Accuracy(ACC) by nearly 1 score on average compared to existing SOTA merging methods, thereby establishing a more favorable trade-off between safety and performance. Moreover, the consistently superior results independent of the type of backdoor or the number of backdoored models, emphasize the robustness and generalizability of our approach.

In all, our contributions can be concluded as follows:


% The full optimization is achieved without any prior assumptions about the nature of the backdoors, making our method robust and broadly applicable. 


% 最后，summarize our contribution

\begin{itemize}
  \item We conduct extensive experiments to investigate the backdoor effect for multi-task merging and uncover the phenomena of backdoor succession and backdoor transfer in existing model merging techniques, highlighting the need for safety-aware designs during merging.
  \item We propose a novel Defense-Aware Merging algorithm through a dual-mask optimization, which simultaneously mitigates the interference and backdoor issues, ensuring a balance between performance and safety for multi-task merging.
  \item We validate the effectiveness of the proposed method on multiple benchmarks, demonstrating effective and robust defense effects against the backdoor.
\end{itemize}

==> section/2.related_work.tex <==
\section{Related Work}
\subsection{Multi-Task Model Merging}
% The proposal of Linear Model Connectivity \citep{frankle2020linear}, which advocates that the weights from the models sharing a part of the optimization trajectory can be interpolated without reducing the overall utility, has spurred the rapid developments of model merging techniques \citep{izmailov2018averaging,frankle2020linear,ilharco2022patching,yang2024model}. 
Multitask model merging aims to provide cost-effective parameter fusion strategies to integrate multiple task-specific finetuned models from the shared pre-trained model into a unified one that can handle various tasks \citep{tang2024fusionbench,yang2024model}.
% has achieved great attention owing to its independence from training data and superior computational efficiency.
The well-known strategy to merge multiple task-specific models is by performing element-wise interpolation on weights, such as Weight Average \citep{wortsman2022model,kaddour2022stop,chronopoulou2023adaptersoup,sanyal2023understanding,lawson2024merging,jia2024revisiting}, Fisher merging \citep{matena2022merging,ryu2023fisher,nathan2024fisher}, RegMean \citep{jin2022dataless}, and Task Arithmetic \citep{ilharco2022editing,zhang2023composing,ni2023forgetting,ortiz2024task}. To further enhance the effectiveness of merging, many efforts have been devoted to addressing interference among tasks and proposing gradient-conflict-based \citep{yadav2024ties}, representation-based \citep{yang2023adamerging,yang2024representation}, and subspace-based methods \citep{tang2023concrete,tam2024merging,yu2024language}. However, these works aim to facilitate knowledge transfer during model merging, but harmful elements like adversarially injected backdoors may also succeed and transfer. Unfortunately, there is insufficient analysis of how multi-task merging will be affected if one or more task-specific models are injected with the backdoor.

% these works share the same goal to facilitate the transfer and inheritance of knowledge from individual models during merging. Exactly, apart from the useful knowledge, the harmful part from one or more models (e.g. backdoor), which may be intentionally injected by the adversary, can also succeed and transfer during the merging process. \textbf{Unfortunately, there is a lack of comprehensive analysis and discussion on how multi-task merging will be affected if one or more task-specific models are injected with the backdoor.}

\subsection{Model Merging Considering the Safety}
The safety of machine learning algorithms is the key to their widespread applications \citep{wu2022backdoorbench}. Recently, many researchers have begun to emphasize safety concerns associated with merging scenarios \citep{yang2024model}. For example, some works adopt the subspace-based and data-aware merging methods to deal with the misalignment \citep{yi2024safety,hammoud2024model} and Intellectual Property Protection \citep{cong2024have} problems for large language models (LLMs). Consistent with our work that focuses on the backdoor issues, WAG \citep{arora2024here} and LoRA-as-an-Attack \citep{liu2024lora} conducted preliminary exploration under backdoor defense scenarios. However, they only adopt the initial weight average strategy \citep{wortsman2022model}, to cope with the backdoor issues on the same task without more fine-grained designs(e.g. subspace). Besides, BadMerging \citep{zhang2024badmerging} only focuses on executing effective backdoor attacks to maximize the ASR to break the safeguard for multi-task merging methods, while we mainly consider the defense strategy to minimize the ASR during merging. To the best of our knowledge, our work is the first to conduct extensive experiments to investigate the backdoor effect for multi-task merging scenarios and provide a novel defense-aware merging algorithm to alleviate this problem.


% In detail, WAG \citep{arora2024here} focuses on directly averaging the parameters from the homogeneous models on the same task in addressing the backdoor issues, while we explore the backdoor effect for multi-task merging and provide a subspace-based method to address this problem; LoRA-as-an-Attack \citep{liu2024lora} proposes to arrange every task with a proper defense Lora and average their weights to weaken the backdoor effect, this may be impractical when we can not know the backdoor types and whether the models that need merging are safe or not in advance. 




% One of the typical safety issues is backdoor learning, which could insert an imperceptible backdoor into the model by maliciously manipulating the training data or controlling the training process \citep{wu2022backdoorbench}.
% For model merging \citep{yang2024model}, the consideration about the safety can be categorized into: 


% \textbf{(i) Utilizing the Existing Merging Techniques to Address the Safety Problem:} These works deploy existing merging methods in various specific circumstances. 


% For example, WAG \citep{arora2024here} utilizes the Weight Average strategy to merge models with different types of attack on the same task to sanitize the backdoor; OTBR \citep{lin2024fusing} adopts the optimal transport-based merging strategy to merge backdoor models and pruned models to achieve a model with high clean accuracy and a low attack success rate on a given specific task; 



% SOMF \citep{yi2024safety}, EvoMM \citep{hammoud2024model} and MergeGuard \citep{cong2024have} respectively adopt the concrete subspace and data-aware merging methods to deal with the misalignment and Intellectual Property Protection problems for large language models (LLMs). Neither of these works considers the safety issue of the merging techniques themselves.



% \textbf{(ii) The Potential Safety Risks of Model Merging Techniques Themselves: These works are most related to ours that focus on the backdoor succession and transfer during merging, especially when one or more task-specific models we would like to merge may be injected backdoor under the share-and-play scenario but we have no access to the training data and the information on whether the models need merging are safe or not.} The latest representative works are LoRA-as-an-Attack \citep{liu2024lora} and BadMerging \citep{zhang2024badmerging}. However, the LoRA-as-an-Attack just provides the experiments of Weight Average using backdoor Lora and defense Lora without other more effective merging strategies. More importantly, it's not practical to arrange every task with a proper defense Lora when we can not know the backdoor types and whether the models that need merging are safe or not in advance. Besides, as a contemporary work, BadMerging only focuses on the backdoor attack to break the safeguard for existing merging methods rather than considering the defense strategy during merging.

